Unifying the Perspectives of NLP and Software Engineering: A Survey on Language Models for Code

In this work we systematically review the recent advancements in software engineering with language models, covering 70+ models, 40+ evaluation tasks, 180+ datasets, and 900 related works. Unlike previous works, we integrate software engineering (SE) with natural language processing (NLP) by discussing the perspectives of both sides: SE applies language models for development automation, while NLP adopts SE tasks for language model evaluation. We break down code processing models into general language models represented by the GPT family and specialized models that are specifically pretrained on code, often with tailored objectives. We discuss the relations and differences between these models, and highlight the historical transition of code modeling from statistical models and RNNs to pretrained Transformers and LLMs, which is exactly the same course that had been taken by NLP. We also go beyond programming and review LLMs' application in other software engineering activities including requirement engineering, testing, deployment, and operations in an endeavor to provide a global view of NLP in SE, and identify key challenges and potential future directions in this domain. We keep the survey open and updated on GitHub at https://github.com/codefuse-ai/Awesome-Code-LLM.

==> trees/task1-text2code.tex <==
\begin{forest}
for tree={
forked edges,
draw,
rounded corners,
grow=east,
anchor=base west,
anchor=center,
reversed=true,
l sep=0.2cm,
},
where level=0{font=\tiny}{},
where level=1{text width=4.9em,font=\tiny}{},
where level=2{text width=3.5em,font=\tiny}{},
where level=3{text width=6em,font=\tiny}{},
where level=4{text width=8em,font=\tiny}{},
where level=5{text width=13em,font=\tiny}{},
for tree={
  if level=0{l sep+=0.15cm}{},
  if level=1{l sep+=0.15cm}{},
  if level=2{l sep+=0.03cm}{},
},
[Code Evaluation, fill=black, fill opacity=0.7, text=white
    [Text-to-Code, fill=yellow, fill opacity=0.5
        [Math Programming, fill=yellow, fill opacity=0.5
            [, fill=yellow, fill opacity=0.5
                [, fill=yellow, fill opacity=0.5
                    [
                    , fill=yellow, fill opacity=0.5
                    ]
                ]
            ]
        ]
    ]
    [Code-to-Code, fill=cyan, fill opacity=0.2]
    [Code-to-Text, fill=Orange, fill opacity=0.2]
    [Code-to-Pattern, fill=VioletRed, fill opacity=0.2]
    [Text-to-Text, fill=Dandelion, fill opacity=0.4]
]
\end{forest}


==> trees/task2-code2code.tex <==
\begin{forest}
for tree={
forked edges,
draw,
rounded corners,
grow=east,
anchor=base west,
anchor=center,
reversed=true,
l sep=0.2cm,
},
where level=0{font=\tiny}{},
where level=1{text width=4.9em,font=\tiny}{},
where level=2{text width=3.5em,font=\tiny}{},
where level=3{text width=8em,font=\tiny}{},
where level=4{text width=8em,font=\tiny}{},
where level=5{text width=11em,font=\tiny}{},
for tree={
  if level=0{l sep+=0.15cm}{},
  if level=1{l sep+=0.15cm}{},
  if level=2{l sep+=0.03cm}{},
},
[Code Evaluation, fill=black, fill opacity=0.7, text=white
    [Text-to-Code, fill=yellow, fill opacity=0.5
    ]
    [Code-to-Code, fill=cyan, fill opacity=0.2
    ]
    [Code-to-Text, fill=Orange, fill opacity=0.2]
    [Code-to-Pattern, fill=VioletRed, fill opacity=0.2]
    [Text-to-Text, fill=Dandelion, fill opacity=0.4]
]
\end{forest}


==> trees/task2-code2code2.tex <==
\begin{forest}
for tree={
forked edges,
draw,
rounded corners,
grow=east,
anchor=base west,
anchor=center,
reversed=true,
l sep=0.2cm,
},
where level=0{font=\tiny}{},
where level=1{text width=4.9em,font=\tiny}{},
where level=2{text width=4.1em,font=\tiny}{},
where level=3{text width=10em,font=\tiny}{},
where level=4{text width=6em,font=\tiny}{},
where level=5{text width=11em,font=\tiny}{},
for tree={
  if level=0{l sep+=0.15cm}{},
  if level=1{l sep+=0.15cm}{},
  if level=2{l sep+=0.03cm}{},
},
[Code Evaluation, fill=black, fill opacity=0.7, text=white
    [Text-to-Code, fill=yellow, fill opacity=0.5
    ]
    [Code-to-Code, fill=cyan, fill opacity=0.2
    ]
    [Code-to-Text, fill=Orange, fill opacity=0.2]
    [Code-to-Pattern, fill=VioletRed, fill opacity=0.2]
    [Text-to-Text, fill=Dandelion, fill opacity=0.4]
]
\end{forest}


==> trees/task3-code2text.tex <==
\begin{forest}
for tree={
forked edges,
draw,
rounded corners,
grow=east,
anchor=base west,
anchor=center,
reversed=true,
l sep=0.2cm,
},
where level=0{font=\tiny}{},
where level=1{text width=4.9em,font=\tiny}{},
where level=2{text width=3.5em,font=\tiny}{},
where level=3{text width=7em,font=\tiny}{},
where level=4{text width=9em,font=\tiny}{},
where level=5{text width=11em,font=\tiny}{},
for tree={
  if level=0{l sep+=0.15cm}{},
  if level=1{l sep+=0.15cm}{},
  if level=2{l sep+=0.03cm}{},
},
[Code Evaluation, fill=black, fill opacity=0.7, text=white
    [Text-to-Code, fill=yellow, fill opacity=0.5]
    [Code-to-Code, fill=cyan, fill opacity=0.2]
    [Code-to-Text, fill=Orange, fill opacity=0.2
    ]
    [Code-to-Pattern, fill=VioletRed, fill opacity=0.2
    ]
    [Text-to-Text, fill=Dandelion, fill opacity=0.4
    ]
]
\end{forest}


==> trees/task4-code2pattern.tex <==
\begin{forest}
for tree={
forked edges,
draw,
rounded corners,
grow=east,
anchor=base west,
anchor=center,
reversed=true,
l sep=0.2cm,
},
where level=0{font=\tiny}{},
where level=1{text width=4.9em,font=\tiny}{},
where level=2{text width=4.1em,font=\tiny}{},
where level=3{text width=6em,font=\tiny}{},
where level=4{text width=10em,font=\tiny}{},
where level=5{text width=11em,font=\tiny}{},
for tree={
  if level=0{l sep+=0.15cm}{},
  if level=1{l sep+=0.15cm}{},
  if level=2{l sep+=0.03cm}{},
},
[Code Evaluation, fill=black, fill opacity=0.7, text=white
    [Text-to-Code, fill=yellow, fill opacity=0.5]
    [Code-to-Code, fill=cyan, fill opacity=0.2]
    [Code-to-Text, fill=Orange, fill opacity=0.2]
    [Code-to-Pattern, fill=VioletRed, fill opacity=0.2
    ]
    [Text-to-Text, fill=Dandelion, fill opacity=0.4
    ]
]
\end{forest}

